Approximate the individually fair k-center with outliers

In this paper, we propose and investigate the individually fair $k$-center with outliers (IF$k$CO). In the IF$k$CO, we are given an $n$-sized vertex set in a metric space, as well as integers $k$ and $q$. At most $k$ vertices can be selected as the centers and at most $q$ vertices can be selected as the outliers. The centers are selected to serve all the not-an-outlier (i.e., served) vertices. The so-called individual fairness constraint restricts that every served vertex must have a selected center not too far way. More precisely, it is supposed that there exists at least one center among its $\lceil (n-q) / k \rceil$ closest neighbors for every served vertex. Because every center serves $(n-q) / k$ vertices on the average. The objective is to select centers and outliers, assign every served vertex to some center, so as to minimize the maximum fairness ratio over all served vertices, where the fairness ratio of a vertex is defined as the ratio between its distance with the assigned center and its distance with a $\lceil (n - q )/k \rceil_{\rm th}$ closest neighbor. As our main contribution, a 4-approximation algorithm is presented, based on which we develop an improved algorithm from a practical perspective.

==> jogobibfile.tex <==

@inproceedings{abv,
  title={Fair clustering via equitable group representations},
  author={Abbasi, Mohsen and Bhaskara, Aditya and Venkatasubramanian, Suresh},
  booktitle={Proceedings of the 2021 ACM Conference on Fairness, Accountability, and Transparency},
  pages={504--514},
  year={2021}
}

@inproceedings{aekm,
  title={Clustering without over-representation},
  author={Ahmadian, Sara and Epasto, Alessandro and Kumar, Ravi and Mahdian, Mohammad},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={267--275},
  year={2019}
}


@inproceedings{biosvw,
  title={Scalable fair clustering},
  author={Backurs, Arturs and Indyk, Piotr and Onak, Krzysztof and Schieber, Baruch and Vakilian, Ali and Wagner, Tal},
  booktitle={Proceedings of the 36th International Conference on Machine Learning},
  pages={405--413},
  year={2019}
}

@inproceedings{bcfn,
  title={Fair algorithms for clustering},
  author={Bera, Suman K and Chakrabarty, Deeparnab and Flores, Nicolas J and Negahbani, Maryam},
  booktitle={Proceedings of the 33rd Annual Conference on Neural Information Processing Systems},
  pages={4954--4965},
  year={2019}
}

@article{bgkkrss,
  title={On the cost of essentially fair clusterings},
  author={Bercea, Ioana O and Gro{\ss}, Martin and Khuller, Samir and Kumar, Aounon and R{\"o}sner, Clemens and Schmidt, Daniel R and Schmidt, Melanie},
  journal={arXiv preprint arXiv:1811.10319},
  year={2018}
}


@inproceedings{bprst,
  title={An improved approximation for $k$-median, and positive correlation in budgeted optimization},
  author={Byrka, Jaros{\l}aw and Pensyl, Thomas and Rybicki, Bartosz and Srinivasan, Aravind and Trinh, Khoa},
  booktitle={Proceedings of the 26th annual ACM-SIAM symposium on Discrete algorithms},
  pages={737--756},
  year={2014}
}

@article{cgts,
  title={A constant-factor approximation algorithm for the $k$-median problem},
  author={Charikar, Moses and Guha, Sudipto and Tardos, {\'E}va and Shmoys, David B},
  journal={Journal of Computer and System Sciences},
  volume={65},
  number={1},
  pages={129--149},
  year={2002},
  publisher={Elsevier}
}

@inproceedings{cklv,
  title={Fair Clustering Through Fairlets},
  author={Chierichetti, Flavio and Kumar, Ravi and Lattanzi, Silvio and Vassilvitskii, Sergei},
  booktitle={Proceedings of the 31st Annual Conference on Neural Information Processing Systems},
  pages={5036--5044},
  year={2017}
}


@inproceedings{c,
  title={Approximation schemes for capacitated clustering in doubling metrics},
  author={Cohen-Addad, Vincent},
  booktitle={Proceedings of the 14th Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={2241--2259},
  year={2020}
}

@inproceedings{gsv,
  title={Socially fair $k$-means clustering},
  author={Ghadiri, Mehrdad and Samadi, Samira and Vempala, Santosh},
  booktitle={Proceedings of the 2021 ACM Conference on Fairness, Accountability, and Transparency},
  pages={438--448},
  year={2021}
}

@article{g,
  title={Clustering to minimize the maximum intercluster distance},
  author={Gonzalez, Teofilo F},
  journal={Theoretical computer science},
  volume={38},
  pages={293--306},
  year={1985},
  publisher={Elsevier}
}

@inproceedings{hjv,
  title={Coresets for clustering with fairness constraints},
  author={Huang, Lingxiao and Jiang, Shaofeng H-C and Vishnoi, Nisheeth K},
  booktitle={Proceedings of the 33rd Annual Conference on Neural Information Processing Systems},
  pages={7589--7600},
  year={2019}
}

@article{hs85,
  title={A best possible heuristic for the k-center problem},
  author={Hochbaum, Dorit S and Shmoys, David B},
  journal={Mathematics of operations research},
  volume={10},
  number={2},
  pages={180--184},
  year={1985},
  publisher={INFORMS}
}

@article{hs86,
  title={A unified approach to approximation algorithms for bottleneck problems},
  author={Hochbaum, Dorit S and Shmoys, David B},
  journal={Journal of the ACM},
  volume={33},
  number={3},
  pages={533--550},
  year={1986},
  publisher={ACM New York}
}

@inproceedings{jnn,
  title={Fair $k$-centers via maximum matching},
  author={Jones, Matthew and Nguyen, Huy and Nguyen, Thy},
  booktitle={International Conference on Machine Learning},
  pages={4940--4949},
  year={2020}
}

@article{jkl,
  title={Service in your neighborhood: Fairness in center location},
  author={Jung, Christopher and Kannan, Sampath and Lutz, Neil},
  journal={Foundations of Responsible Computing},
  year={2020}
}



@article{kps,
  title={Fault tolerant k-center problems},
  author={Khuller, Samir and Pless, Robert and Sussmann, Yoram J},
  journal={Theoretical Computer Science},
  volume={242},
  number={1-2},
  pages={237--245},
  year={2000},
  publisher={Elsevier}
}


@article{ks,
  title={The capacitated k-center problem},
  author={Khuller, Samir and Sussmann, Yoram J},
  journal={SIAM Journal on Discrete Mathematics},
  volume={13},
  number={3},
  pages={403--418},
  year={2000},
  publisher={SIAM}
}


@inproceedings{kam,
  title={Fair $k$-center clustering for data summarization},
  author={Kleindessner, Matth{\"a}us and Awasthi, Pranjal and Morgenstern, Jamie},
  booktitle={Proceedings of the 36th International Conference on Machine Learning},
  pages={3448--3457},
  year={2019}
}

@inproceedings{kls,
  title={Constant approximation for $k$-median and k-means with outliers via iterative rounding},
  author={Krishnaswamy, Ravishankar and Li, Shi and Sandeep, Sai},
  booktitle={Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={646--659},
  year={2018}
}

@article{l,
  title={A 1.488 approximation algorithm for the uncapacitated facility location problem},
  author={Li, Shi},
  journal={Information and Computation},
  volume={222},
  pages={45--58},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{mvi,
  title={Individual fairness for $k$-clustering},
  author={Mahabadi, Sepideh and Vakilian, Ali},
  booktitle={Proceedings of the 37th International Conference on Machine Learning},
  pages={6586--6596},
  year={2020},
  organization={PMLR}
}

@article{mv,
  title={Approximation Algorithms for Socially Fair Clustering},
  author={Makarychev, Yury and Vakilian, Ali},
  journal={arXiv preprint arXiv:2103.02512},
  year={2021}
}

@inproceedings{sss,
  title={Fair coresets and streaming algorithms for fair $k$-means},
  author={Schmidt, Melanie and Schwiegelshohn, Chris and Sohler, Christian},
  booktitle={Proceedings of the 17th International Workshop on Approximation and Online Algorithms},
  pages={232--251},
  year={2019}
}

@inproceedings{sta,
  title={Approximation algorithms for facility location problems},
  author={Shmoys, David B and Tardos, {\'E}va and Aardal, Karen},
  booktitle={Proceedings of the 29th annual ACM symposium on Theory of computing},
  pages={265--274},
  year={1997}
}

@article{vy,
  title={Improved approximation algorithms for individually fair clustering},
  author={Vakilian, Ali and Yal{\c{c}}{\i}ner, Mustafa},
  journal={arXiv preprint arXiv:2106.14043},
  year={2021}
}


@article{xxdw,
  title={Local search algorithm for universal facility location problem with linear penalties},
  author={Xu, Yicheng and Xu, Dachuan and Du, Donglei and Wu, Chenchen},
  journal={Journal of Global Optimization},
  volume={67},
  number={1-2},
  pages={367--378},
  year={2017},
  publisher={Springer}
}

@article{xxzz,
  title={MpUFLP: Universal facility location problem in the $p$-th power of metric space},
  author={Xu, Yicheng and Xu, Dachuan and Zhang, Yong and Zou, Juan},
  journal={Theoretical Computer Science},
  volume={838},
  pages={58--67},
  year={2020},
  publisher={Elsevier}
}


@misc{link,
  title = {{Gaode Maps},
  {\url{https://lbs.amap.com/api/webservice/guide/api/ipconfig}}
}
%\bibitem{link}
%\url{https://lbs.amap.com/api/webservice/guide/api/ipconfig}

